Morse Theoretic Templates for High Dimensional Homology Computation

We introduce the notion of a template for discrete Morse theory. Templates provide a memory efficient approach to the computation of homological invariants (e.g., homology, persistent homology, Conley complexes) of cell complexes. We demonstrate the effectiveness of templates in two settings: first, by computing the homology of certain cubical complexes which are homotopy equivalent to $\mathbb{S}^d$ for $1\leq d \leq 20$, and second, by computing Conley complexes and connection matrices for a collection of examples arising from a Conley-Morse theory on spaces of braids diagrams.

==> correctm.tex <==
% This file defines a few macros useful in team work on a paper or a book.
% The main purpose of the macros is to faciliate having simultanously two versions
% of selected fragments of text (old and new) with appropriate comments so that
% co-authors may think before deciding which version is better.
%
% To use these macros you must put this file in the directory where you keep
% the source files and add the following two lines
%
%\include{correctm}
%\showcomments
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
%
% at the beginnig of the main source file.
% If you want to compile the source file without any comments,
% just replace \showcomments by \hidecomments. In this case only the new versions
% will be used in the compiled text and all comments will be ommitted.
% This gives a possibility of looking at the clean text while still keeping
% the alternatives in the source file
%
% The \corrl macro
% ================
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
%
% The main macro is \corrl and it has the following syntax
%
% \corrl comment<<old_version||new_version>>
%
% Note that <<, || and >> are obligatory even if old_version or new_version are empty texts.
% The words 'comment', 'old_version', 'new_version',
% mark the places where you put your own text, i.e. these are parameters of the macro.
% The meaning of the parameters is
%
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
%     'comment'     - just a comment set in a non-standard font so that it clearly differs from
%                      the proper text
%     'old_version' - here you put the old text, which you want replaced with the new text
%     'new_version' - here you put the new text
%
% If comments are turned on by \showcomments, you will see the comment, then the old version
% clearly seperated form the new version and a margin mark. If comments are turned off, you
% will see only the new version with no comments or marks.
%
% If comment, old_version and/or new_version are longer than one line, a good idea is
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
% to write this macro (as well as the following macros) as
% \corrl
%   comment
% <<
%   old_version
% ||
%   new_version
% >>
%
%
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
% The \corrq macro
% ================
%
% Another possibility is that you feel some fragment should be changed but you do not know what
% should be the new version. Then use the macro
%
%  \corrq comment<<questioned_text>>
%
% With comments turned on you will see the comment followed by the clearly marked
% questioned text
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
%
% The \corre macro
% ================
%
% Sometimes the new version is an almost obvious change, so you
% want the old version only in the source
% file (just in case ...) but not in the compiled file.
% Then use the macro
%
% \corre comment<<old_version||new_version>>
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
%
% which in the compiled file shows only the new version and the margin mark to indicate that
% changes were made.
%
% The \corrs macro
% ================
%
% When the change is almost obvious and short, use the macro
%
% \corrs comment<<old_version||new_version>>
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
%
% which is similar to the previous but automaticallly adds a comment
% old_version->new_version on the margin
%
% The \corrn and \corro macros
% ============================
%
% To settle matters you can use two more macros with the same syntax as \corrl
%
%  \corro - to force the old version - the new version and all comments are disregarded
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
%                                      (but present in the source file)
%  \corrn - to force the new version - the old version and all comments are disregarded
%                                      (but present in the source file)
%
% This is simple in use (just replace l, q or s in the macro name by o or n) but leaves rubbish
% in the source file. If you find ourselve using plenty of this stuff one can easily write a simple PERL
% script which will automatically remove all this rubbish.
%
%
% The \corrc macro
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
% ================
%
% This is to place in the source file a comment only. The syntax is
%
% \corrc comment <<>>
%
% Parameters containing whole paragraphs
% ======================================
%
% Note: the standard TeX macros cannot be called with parameters which go across paragraphs
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
% (i.e. contain \par or an empty line). However, there is a special mechanism which allows for that.
% It is implemented here in the form of alternative macros \longcorrl, \longcorrq, \longcorrs and so on.
% Since TeX better recovers from errors if such macros are not present, use them only when necessary.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Macro definitions %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\def\corcommstyle{\bf\tiny}
\def\corcommstyle{\bf\small\tt}

%This macro is to be used when an alternative approach is to be displayed
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
%versus the old approach

\def\corrl #1<<#2||#3>>{
\if\visiblecomments y
  \begin{quote} {\corcommstyle $<<$COMMENT$>>$ {\color{red}#1\marginpar{!!}}\\$<<$OLD$<<$} \end{quote}

{\color{red} #2 }
 
 

  \begin{quote} {\corcommstyle ==NEW== } \end{quote}
   \noindent\hrulefill
 
\vspace{-10pt} 
 
 \noindent\hrulefill
 
 \vspace{-10pt} 
 
 \noindent\dotfill
 
  #3
  
   \noindent\dotfill 

\vspace{-10pt} 
 
 \noindent\hrulefill
 
 \vspace{-10pt} 
 
 \noindent\hrulefill
  \begin{quote} {\corcommstyle $>>$END$>>$ } \end{quote}
 \else
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
  #3
 \fi
}

\long\def\longcorrl #1<<#2||#3>>{
\if\visiblecomments y
  \begin{quote} {\corcommstyle $<<$COMMENT$>>$ {\color{red}#1\marginpar{!!}}\\$<<$OLD$<<$} \end{quote}
 
 {

  #2
  
  }
  
  \begin{quote} {\corcommstyle ==NEW== } \end{quote}
  
    \noindent\hrulefill
 
\vspace{-10pt} 
 
 \noindent\hrulefill
 
 \vspace{-10pt} 
 
 \noindent\dotfill
 
  #3
  
   \noindent\dotfill 

\vspace{-10pt} 
 
 \noindent\hrulefill
 
 \vspace{-10pt} 
 
 \noindent\hrulefill
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
  \begin{quote} {\corcommstyle $>>$END$>>$ } \end{quote}
 \else
  #3
 \fi
}

\def\mlabel #1
{
  \if\visiblecomments y
     \marginpar[\flushright \bf \footnotesize #1]{\bf \footnotesize #1}
  \fi
}

\def\flabel #1
{
  \if\visiblecomments y
       \hbox{\bf\footnotesize #1}
  \fi
}


%This macro is to be used when there is some confusion
%No new text is proposed

%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
\def\corrq #1<<#2>>{
\if\visiblecomments y
  \begin{quote} {\corcommstyle $<<$COMMENT$>>$ #1\marginpar{!!}\\$<<$BEG$<<$} \end{quote}
  \noindent\hrulefill
 
\vspace{-10pt} 
 
 \noindent\hrulefill
 
 \vspace{-10pt} 
 
 \noindent\dotfill
 
 {\color{red}
  
  #2
  
  }
   
  \noindent\dotfill 

\vspace{-10pt} 
 
 \noindent\hrulefill
 
 \vspace{-10pt} 
 
 \noindent\hrulefill 
  \begin{quote} {\corcommstyle $>>$END$>>$ } \end{quote}
 \else
  #2
 \fi
}

%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
\long\def\longcorrq #1<<#2>>{
\if\visiblecomments y
  \begin{quote} {\corcommstyle $<<$COMMENT$>>$ #1\marginpar{!!}\\$<<$BEG$<<$} \end{quote}
  \noindent\hrulefill
 
\vspace{-10pt} 
 
 \noindent\hrulefill
 
 \vspace{-10pt} 
 
 \noindent\dotfill

  #2

  \noindent\dotfill 

\vspace{-10pt} 
 
 \noindent\hrulefill
 
 \vspace{-10pt} 
 
 \noindent\hrulefill 
  \begin{quote} {\corcommstyle $>>$END$>>$ } \end{quote}
 \else
  #2
 \fi
}

%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
%This is just to introduce a comment

\def\corrc #1<<>>{
\if\visiblecomments y
  \begin{quote} {\corcommstyle $<<$COMMENT$>>$ \color{red} #1\marginpar{!!}} \end{quote}
\fi
}

%This macro is intended for some evident corrections.
%Only the new text is displayed.
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
%Comment is typed on the margin.

\def\corre #1<<#2||#3>>{
\if\visiblecomments y
  #3\marginpar{\corcommstyle #1}
 \else
  #3
 \fi
}

%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
\long\def\longcorre #1<<#2||#3>>{
\if\visiblecomments y
  #3\marginpar{\corcommstyle #1}
 \else
  #3
 \fi
}

%This macro is intended to mark corrections to short simple typos.
%Only the new text is displayed and an automatic typo change is
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
%marked on the margin.

\def\corrs #1<<#2||#3>>{
\if\visiblecomments y
  #3\marginpar{\corcommstyle #2 $\rightarrow$ #3\\ #1}
 \else
  #3
 \fi
}

%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
%The next two macros are to help settle the matters.
%Changing \corrx where x is l,q or s to \corro (\corrn)
%will result in just choosing the old (new) text.
%This is intended to provide a simple way to get rid of
%any comments, i.e. to "clean" the paper.
%Unfortunately the no longer needed versions remain
%in the source file so in the future it would be
%useful to have some preprocessor to clean also
%the source file.
%Note that since \corrq does not provide any new stuff
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
%it makes sense only to change it to \corro unless some
%new text is added later on.

\def\corro #1<<#2||#3>>{
#2}

\def\corrn #1<<#2||#3>>{
#3}

\long\def\longcorro #1<<#2||#3>>{
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
#2}

\long\def\longcorrn #1<<#2||#3>>{
#3}

% This macro is to hide in official version pieces of text
% which is not available for presentation yet.

\long\def\underconstruction #1<<<#2>>>{
\if\visiblecomments y
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
  \begin{quote} {\corcommstyle $<<$UNDER CONSTRUCTION - BEGIN$>>$ #1\marginpar{!!}} \end{quote}
   {\color{red}
  #2
  }
  \begin{quote} {\corcommstyle $>>$UNDER CONSTRUCTION - END$>>$ } \end{quote}
 \else
 \fi
}



% These two macros are to tourn on/off comments
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%

\def\showcomments{
  \let\visiblecomments y
}

\def\hidecomments{
  \let\visiblecomments n
}


%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%


